Smoothing for signals with discontinuities using higher order Mumford-Shah models

Minimizing the Mumford-Shah functional is frequently used for smoothing signals or time series with discontinuities. A significant limitation of the standard Mumford-Shah model is that linear trends -- and in general polynomial trends -- in the data are not well preserved. This can be improved by building on splines of higher order which leads to higher order Mumford-Shah models. In this work, we study these models in the univariate situation: we discuss important differences to the first order Mumford-Shah model, and we obtain uniqueness results for their solutions. As a main contribution, we derive fast minimization algorithms for Mumford-Shah models of arbitrary orders. We show that the worst case complexity of all proposed schemes is quadratic in the length of the signal. Remarkably, they thus achieve the worst case complexity of the fastest solver for the piecewise constant Mumford-Shah model (which is the simplest model of the class). Further, we obtain stability results for the proposed algorithms. We complement these results with a numerical study. Our reference implementation processes signals with more than 10,000 elements in less than one second.

==> Experiments/Parameter_Choice/Elasticity_A/Elasticity_1.tex <==
\begin{figure}[H]
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Parameter_Choice/Elasticity_A/Elasticity_1.pdf}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Parameter_Choice/Elasticity_A/Elasticity_2.pdf}
	\end{subfigure}\\[1em]
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Parameter_Choice/Elasticity_A/Elasticity_3.pdf}
	\end{subfigure}
	\caption{
	Role of elasticity parameter $\alpha$ for fixed
	$\gamma=\protect\input{Experiments/Parameter_Choice/Elasticity_A/gamma_1.tex},~ k=\protect\input{Experiments/Parameter_Choice/Elasticity_A/k_1.tex}$.
	Upper left: $\alpha=\protect\input{Experiments/Parameter_Choice/Elasticity_A/alpha_1.tex}
	$.
	Upper right: 
	$\alpha=\protect\input{Experiments/Parameter_Choice/Elasticity_A/alpha_2.tex}
	$.
	Bottom: 
	$\alpha=\protect\input{Experiments/Parameter_Choice/Elasticity_A/alpha_3.tex}
	$.
		}

\end{figure}

==> Experiments/Parameter_Choice/Elasticity_A/alpha_1.tex <==
0.5

==> Experiments/Parameter_Choice/Elasticity_A/alpha_2.tex <==
100

==> Experiments/Parameter_Choice/Elasticity_A/alpha_3.tex <==
5000

==> Experiments/Parameter_Choice/Elasticity_A/gamma_1.tex <==
1

==> Experiments/Parameter_Choice/Elasticity_A/gamma_2.tex <==
1

==> Experiments/Parameter_Choice/Elasticity_A/gamma_3.tex <==
1

==> Experiments/Parameter_Choice/Elasticity_A/k_1.tex <==
3

==> Experiments/Parameter_Choice/Elasticity_A/k_2.tex <==
3

==> Experiments/Parameter_Choice/Elasticity_A/k_3.tex <==
3

==> Experiments/Parameter_Choice/Elasticity_B/Elasticity_B_Data.tex <==
\begin{figure}[]
	\centering
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{Experiments/Parameter_Choice/Elasticity_B/Groundtruth.pdf}
\subcaption{\label{Fig Mallat groundtruth}}
\end{subfigure}\\[1em]
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{Experiments/Parameter_Choice/Elasticity_B/Noisy_01.pdf}
\subcaption{\label{Fig Mallat nlvl_1}
	}
\end{subfigure}~
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{Experiments/Parameter_Choice/Elasticity_B/Noisy_02.pdf}
\subcaption{\label{Fig Mallat nlvl_2}
	}
\end{subfigure}~
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\textwidth]{Experiments/Parameter_Choice/Elasticity_B/Noisy_03.pdf}
\subcaption{\label{Fig Mallat nlvl_3}
	}
\end{subfigure}
\caption{
	\label{Fig Elasticity Data}
	Reference signal \eqref{Fig Mallat groundtruth} and data corrupted by increasing noise levels $\eta$.
	\eqref{Fig Mallat nlvl_1}: $\eta = \protect\input{Experiments/Parameter_Choice/Elasticity_B/nlvl_01.tex}$.
	\eqref{Fig Mallat nlvl_2}: $\eta = \protect\input{Experiments/Parameter_Choice/Elasticity_B/nlvl_02.tex}$.
	\eqref{Fig Mallat nlvl_3}: $\eta = \protect\input{Experiments/Parameter_Choice/Elasticity_B/nlvl_03.tex}$.
}
\end{figure}

==> Experiments/Parameter_Choice/Elasticity_B/Elasticity_B_Table.tex <==
\begin{table}[!t]	
\centering
\small
\begin{tabular}{ l  r  r  r  r  r}
\toprule
% \multicolumn{6}{c}{Noise$\qquad\qquad\qquad\qquad \quad k\qquad\qquad\qquad\qquad$} 
%\multirow{7	}*{\rotatebox{90}{Noise level$\quad$}}
\input{Experiments/Parameter_Choice/Elasticity_B/Optimal_Elasticity_Table.tex}
\bottomrule
\end{tabular}$\qquad$
\begin{tabular}{ l  r  r  r  r  r}
\toprule
\input{Experiments/Parameter_Choice/Elasticity_B/Optimal_Elasticity_Table_RandIndex.tex} 
\bottomrule
\end{tabular}
\caption{\label{Table Optimal Elasticities}
	Optimal elasticities $\beta$ for various spline orders $k$ and noise levels for the reference signal from
	\cref{Fig Mallat Reconstructions}.
	\emph{Left:} Optimal values with respect to the relative $\ell_2$-error. \emph{Right:} Optimal values with respect to the Rand index of the computed segmentations.
	}
\end{table}


==> Experiments/Parameter_Choice/Elasticity_B/K.tex <==
1, 2, 3, 4, 5

==> Experiments/Parameter_Choice/Elasticity_B/Optimal_Elasticity_Table.tex <==
Noise &  &  & $k$ &  & \\ 
level & 1  & 2  & 3  & 4  & 5 \\ 
 \midrule    
 0.05  & 0.96 & 3.28 & 6.06 & 8.96 & 11.15\\ 
 0.10  & 1.44 & 4.24 & 8.16 & 11.44 & 13.85\\ 
 0.15  & 1.92 & 4.96 & 9.54 & 12.32 & 6.60\\ 
 0.20  & 2.24 & 5.92 & 11.04 & 6.32 & 7.60\\ 
 0.25  & 2.40 & 6.16 & 7.02 & 8.00 & 9.80\\ 
 0.30  & 2.88 & 6.96 & 8.04 & 9.28 & 11.50\\ 


==> Experiments/Parameter_Choice/Elasticity_B/Optimal_Elasticity_Table_RandIndex.tex <==
Noise &  &  & $k$ &  & \\ 
level & 1  & 2  & 3  & 4  & 5 \\ 
 \midrule    
 0.05  & 0.80 & 2.96 & 4.56 & 4.72 & 5.90\\ 
 0.10  & 1.28 & 4.80 & 6.96 & 16.24 & 8.70\\ 
 0.15  & 1.76 & 6.80 & 13.98 & 10.80 & 11.85\\ 
 0.20  & 2.08 & 8.72 & 16.20 & 19.92 & 13.75\\ 
 0.25  & 2.56 & 10.40 & 19.86 & 12.92 & 14.85\\ 
 0.30  & 2.88 & 11.28 & 20.64 & 13.40 & 15.75\\ 


==> Experiments/Parameter_Choice/Elasticity_B/alpha_tick_1.tex <==
0.16

==> Experiments/Parameter_Choice/Elasticity_B/alpha_tick_2.tex <==
0.08

==> Experiments/Parameter_Choice/Elasticity_B/alpha_tick_3.tex <==
0.06

==> Experiments/Parameter_Choice/Elasticity_B/alpha_tick_4.tex <==
0.04

==> Experiments/Parameter_Choice/Elasticity_B/alpha_tick_5.tex <==
0.05

==> Experiments/Parameter_Choice/Elasticity_B/alpha_top_1.tex <==
80

==> Experiments/Parameter_Choice/Elasticity_B/alpha_top_2.tex <==
40

==> Experiments/Parameter_Choice/Elasticity_B/alpha_top_3.tex <==
30

==> Experiments/Parameter_Choice/Elasticity_B/alpha_top_4.tex <==
20

==> Experiments/Parameter_Choice/Elasticity_B/alpha_top_5.tex <==
25

==> Experiments/Parameter_Choice/Elasticity_B/beta_10_1.tex <==
4.724

==> Experiments/Parameter_Choice/Elasticity_B/beta_10_2.tex <==
7.293

==> Experiments/Parameter_Choice/Elasticity_B/beta_10_3.tex <==
13.459

==> Experiments/Parameter_Choice/Elasticity_B/beta_1_1.tex <==
1.175

==> Experiments/Parameter_Choice/Elasticity_B/beta_1_2.tex <==
2.025

==> Experiments/Parameter_Choice/Elasticity_B/beta_1_3.tex <==
3.525

==> Experiments/Parameter_Choice/Elasticity_B/beta_2_1.tex <==
3.625

==> Experiments/Parameter_Choice/Elasticity_B/beta_2_2.tex <==
2.950

==> Experiments/Parameter_Choice/Elasticity_B/beta_2_3.tex <==
8.725

==> Experiments/Parameter_Choice/Elasticity_B/beta_3_1.tex <==
5.350

==> Experiments/Parameter_Choice/Elasticity_B/beta_3_2.tex <==
4.850

==> Experiments/Parameter_Choice/Elasticity_B/beta_3_3.tex <==
7.350

==> Experiments/Parameter_Choice/Elasticity_B/beta_4_1.tex <==
9.725

==> Experiments/Parameter_Choice/Elasticity_B/beta_4_2.tex <==
5.225

==> Experiments/Parameter_Choice/Elasticity_B/beta_4_3.tex <==
8.325

==> Experiments/Parameter_Choice/Elasticity_B/beta_5_1.tex <==
12.625

==> Experiments/Parameter_Choice/Elasticity_B/beta_5_2.tex <==
6.100

==> Experiments/Parameter_Choice/Elasticity_B/beta_5_3.tex <==
9.550

==> Experiments/Parameter_Choice/Elasticity_B/beta_6_1.tex <==
15.000

==> Experiments/Parameter_Choice/Elasticity_B/beta_6_2.tex <==
7.293

==> Experiments/Parameter_Choice/Elasticity_B/beta_6_3.tex <==
11.917

==> Experiments/Parameter_Choice/Elasticity_B/beta_7_1.tex <==
4.210

==> Experiments/Parameter_Choice/Elasticity_B/beta_7_2.tex <==
5.238

==> Experiments/Parameter_Choice/Elasticity_B/beta_7_3.tex <==
13.459

==> Experiments/Parameter_Choice/Elasticity_B/beta_8_1.tex <==
4.210

==> Experiments/Parameter_Choice/Elasticity_B/beta_8_2.tex <==
6.266

==> Experiments/Parameter_Choice/Elasticity_B/beta_8_3.tex <==
10.890

==> Experiments/Parameter_Choice/Elasticity_B/beta_9_1.tex <==
4.210

==> Experiments/Parameter_Choice/Elasticity_B/beta_9_2.tex <==
6.266

==> Experiments/Parameter_Choice/Elasticity_B/beta_9_3.tex <==
11.403

==> Experiments/Parameter_Choice/Elasticity_B/beta_max.tex <==
25

==> Experiments/Parameter_Choice/Elasticity_B/beta_min.tex <==
0.025

==> Experiments/Parameter_Choice/Elasticity_B/gamma_10_1.tex <==
0.035

==> Experiments/Parameter_Choice/Elasticity_B/gamma_10_2.tex <==
0.207

==> Experiments/Parameter_Choice/Elasticity_B/gamma_10_3.tex <==
0.379

==> Experiments/Parameter_Choice/Elasticity_B/gamma_1_1.tex <==
0.005

==> Experiments/Parameter_Choice/Elasticity_B/gamma_1_2.tex <==
0.162

==> Experiments/Parameter_Choice/Elasticity_B/gamma_1_3.tex <==
0.318

==> Experiments/Parameter_Choice/Elasticity_B/gamma_2_1.tex <==
0.003

==> Experiments/Parameter_Choice/Elasticity_B/gamma_2_2.tex <==
0.092

==> Experiments/Parameter_Choice/Elasticity_B/gamma_2_3.tex <==
0.126

==> Experiments/Parameter_Choice/Elasticity_B/gamma_3_1.tex <==
0.012

==> Experiments/Parameter_Choice/Elasticity_B/gamma_3_2.tex <==
0.104

==> Experiments/Parameter_Choice/Elasticity_B/gamma_3_3.tex <==
0.289

==> Experiments/Parameter_Choice/Elasticity_B/gamma_4_1.tex <==
0.020

==> Experiments/Parameter_Choice/Elasticity_B/gamma_4_2.tex <==
0.116

==> Experiments/Parameter_Choice/Elasticity_B/gamma_4_3.tex <==
0.288

==> Experiments/Parameter_Choice/Elasticity_B/gamma_5_1.tex <==
0.040

==> Experiments/Parameter_Choice/Elasticity_B/gamma_5_2.tex <==
0.168

==> Experiments/Parameter_Choice/Elasticity_B/gamma_5_3.tex <==
0.307

==> Experiments/Parameter_Choice/Elasticity_B/gamma_6_1.tex <==
0.035

==> Experiments/Parameter_Choice/Elasticity_B/gamma_6_2.tex <==
0.241

==> Experiments/Parameter_Choice/Elasticity_B/gamma_6_3.tex <==
0.379

==> Experiments/Parameter_Choice/Elasticity_B/gamma_7_1.tex <==
0.035

==> Experiments/Parameter_Choice/Elasticity_B/gamma_7_2.tex <==
0.104

==> Experiments/Parameter_Choice/Elasticity_B/gamma_7_3.tex <==
0.379

==> Experiments/Parameter_Choice/Elasticity_B/gamma_8_1.tex <==
0.035

==> Experiments/Parameter_Choice/Elasticity_B/gamma_8_2.tex <==
0.172

==> Experiments/Parameter_Choice/Elasticity_B/gamma_8_3.tex <==
0.310

==> Experiments/Parameter_Choice/Elasticity_B/gamma_9_1.tex <==
0.035

==> Experiments/Parameter_Choice/Elasticity_B/gamma_9_2.tex <==
0.172

==> Experiments/Parameter_Choice/Elasticity_B/gamma_9_3.tex <==
0.345

==> Experiments/Parameter_Choice/Elasticity_B/gamma_max.tex <==
1

==> Experiments/Parameter_Choice/Elasticity_B/gamma_min.tex <==
0.001

==> Experiments/Parameter_Choice/Elasticity_B/k_1.tex <==
1

==> Experiments/Parameter_Choice/Elasticity_B/k_2.tex <==
2

==> Experiments/Parameter_Choice/Elasticity_B/k_3.tex <==
3

==> Experiments/Parameter_Choice/Elasticity_B/k_4.tex <==
4

==> Experiments/Parameter_Choice/Elasticity_B/n.tex <==
1024

==> Experiments/Parameter_Choice/Elasticity_B/nlvl_01.tex <==
0.05

==> Experiments/Parameter_Choice/Elasticity_B/nlvl_02.tex <==
0.15

==> Experiments/Parameter_Choice/Elasticity_B/nlvl_03.tex <==
0.3

==> Experiments/Parameter_Choice/Elasticity_B/noiselvls.tex <==
5.000000e-02, 1.000000e-01, 1.500000e-01, 2.000000e-01, 2.500000e-01, 3.000000e-01

==> Experiments/Parameter_Choice/Elasticity_B/nr_steps.tex <==
1000

==> Experiments/Parameter_Choice/Elasticity_B/repeats.tex <==
100

==> Experiments/Parameter_Choice/Elasticity_B/rerr_10_1.tex <==
0.013

==> Experiments/Parameter_Choice/Elasticity_B/rerr_10_2.tex <==
0.037

==> Experiments/Parameter_Choice/Elasticity_B/rerr_10_3.tex <==
0.074

==> Experiments/Parameter_Choice/Elasticity_B/rerr_1_1.tex <==
0.020

==> Experiments/Parameter_Choice/Elasticity_B/rerr_1_2.tex <==
0.044

==> Experiments/Parameter_Choice/Elasticity_B/rerr_1_3.tex <==
0.077

==> Experiments/Parameter_Choice/Elasticity_B/rerr_2_1.tex <==
0.013

==> Experiments/Parameter_Choice/Elasticity_B/rerr_2_2.tex <==
0.038

==> Experiments/Parameter_Choice/Elasticity_B/rerr_2_3.tex <==
0.060

==> Experiments/Parameter_Choice/Elasticity_B/rerr_3_1.tex <==
0.011

==> Experiments/Parameter_Choice/Elasticity_B/rerr_3_2.tex <==
0.036

==> Experiments/Parameter_Choice/Elasticity_B/rerr_3_3.tex <==
0.055

==> Experiments/Parameter_Choice/Elasticity_B/rerr_4_1.tex <==
0.011

==> Experiments/Parameter_Choice/Elasticity_B/rerr_4_2.tex <==
0.035

==> Experiments/Parameter_Choice/Elasticity_B/rerr_4_3.tex <==
0.054

==> Experiments/Parameter_Choice/Elasticity_B/rerr_5_1.tex <==
0.010

==> Experiments/Parameter_Choice/Elasticity_B/rerr_5_2.tex <==
0.033

==> Experiments/Parameter_Choice/Elasticity_B/rerr_5_3.tex <==
0.054

==> Experiments/Parameter_Choice/Elasticity_B/rerr_6_1.tex <==
0.010

==> Experiments/Parameter_Choice/Elasticity_B/rerr_6_2.tex <==
0.034

==> Experiments/Parameter_Choice/Elasticity_B/rerr_6_3.tex <==
0.057

==> Experiments/Parameter_Choice/Elasticity_B/rerr_7_1.tex <==
0.013

==> Experiments/Parameter_Choice/Elasticity_B/rerr_7_2.tex <==
0.034

==> Experiments/Parameter_Choice/Elasticity_B/rerr_7_3.tex <==
0.061

==> Experiments/Parameter_Choice/Elasticity_B/rerr_8_1.tex <==
0.013

==> Experiments/Parameter_Choice/Elasticity_B/rerr_8_2.tex <==
0.034

==> Experiments/Parameter_Choice/Elasticity_B/rerr_8_3.tex <==
0.068

==> Experiments/Parameter_Choice/Elasticity_B/rerr_9_1.tex <==
0.013

==> Experiments/Parameter_Choice/Elasticity_B/rerr_9_2.tex <==
0.037

==> Experiments/Parameter_Choice/Elasticity_B/rerr_9_3.tex <==
0.070

==> Experiments/Parameter_Choice/Elasticity_B/sigma_1.tex <==
0.015175

==> Experiments/Parameter_Choice/Elasticity_B/sigma_2.tex <==
0.045525

==> Experiments/Parameter_Choice/Elasticity_B/sigma_3.tex <==
0.09105

==> Experiments/Parameter_Choice/Elasticity_C/Elasticity_C.tex <==
% !TEX root = ../../../higherOrderBZ.tex
\begin{figure}[]
	\centering
	\footnotesize
	\begin{subfigure}{0.24\textwidth}
		\subcaption*{small $\beta$}		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=\protect\input{Experiments/Parameter_Choice/Elasticity_C/k_1.tex}$}}}}%
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_1_01.pdf} \\[1em]
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=\protect\input{Experiments/Parameter_Choice/Elasticity_C/k_2.tex}$}}}}%		
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_2_01.pdf} \\[1em]
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=\protect\input{Experiments/Parameter_Choice/Elasticity_C/k_3.tex}$}}}}%		
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_3_01.pdf} \\[1em]
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=\protect\input{Experiments/Parameter_Choice/Elasticity_C/k_4.tex}$}}}}%				
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_4_01.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.24\textwidth}
		\subcaption*{optimized $\beta$}
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_1_02.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_2_02.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_3_02.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_4_02.pdf}
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.24\textwidth}
		\subcaption*{large $\beta$}
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_1_03.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_2_03.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_3_03.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_4_03.pdf} 
	\end{subfigure}
	\hfill
	\begin{subfigure}{0.24\textwidth}
		\subcaption*{$\beta=\infty$ }
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_1_Potts.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_2_Potts.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_3_Potts.pdf} \\[1em]
		\includegraphics[width=1\textwidth,trim=30 15 13 0, clip]{Experiments/Parameter_Choice/Elasticity_C/Recon_4_Potts.pdf}
	\end{subfigure}
	\caption{ \label{Fig Illustration of Alpha}
		Reconstructions from noisy data using Mumford-Shah models up to order four and various choices of $\beta$ including an optimized value with respect to the $\ell_2$--error. 
		The limit case $\beta=\infty$ corresponds to the higher order Potts model, that is, to piecewise estimation by polynomials up to degree $k-1.$
	}
\end{figure}

==> Experiments/Parameter_Choice/Elasticity_C/k_1.tex <==
1

==> Experiments/Parameter_Choice/Elasticity_C/k_2.tex <==
2

==> Experiments/Parameter_Choice/Elasticity_C/k_3.tex <==
3

==> Experiments/Parameter_Choice/Elasticity_C/k_4.tex <==
4

==> Experiments/Parameter_Choice/Elasticity_C/n.tex <==
1001

==> Experiments/Parameter_Choice/Elasticity_C/nlvl.tex <==
0.1

==> Experiments/Parameter_Choice/JumpPenalty_A/JumpPenalty_1.tex <==
\begin{figure}[H]
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Parameter_Choice//JumpPenalty_A/JumpPenalty_1.pdf}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Parameter_Choice//JumpPenalty_A/JumpPenalty_2.pdf}
	\end{subfigure}\\[1em]
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Parameter_Choice//JumpPenalty_A/JumpPenalty_3.pdf}
	\end{subfigure}
	\caption{
	Role of jump penalty $\gamma$.
	Upper left: $\gamma=\protect\input{Experiments/Parameter_Choice/JumpPenalty_A/gamma_1.tex}
	$.
	Upper right: 
	$\gamma=\protect\input{Experiments/Parameter_Choice/JumpPenalty_A/gamma_2.tex}$.
	Bottom: 
	$\gamma=\protect\input{Experiments/Parameter_Choice/JumpPenalty_A/gamma_3.tex}	
	$.
		}

\end{figure}


==> Experiments/Parameter_Choice/JumpPenalty_A/gamma_1.tex <==
0

==> Experiments/Parameter_Choice/JumpPenalty_A/gamma_2.tex <==
1

==> Experiments/Parameter_Choice/JumpPenalty_A/gamma_3.tex <==
15

==> Experiments/Parameter_Choice/SplineOrder_A/alpha_1.tex <==
100

==> Experiments/Parameter_Choice/SplineOrder_A/alpha_2.tex <==
100

==> Experiments/Parameter_Choice/SplineOrder_A/alpha_3.tex <==
100

==> Experiments/Parameter_Choice/SplineOrder_A/gamma_1.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_A/gamma_2.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_A/gamma_3.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_A/k_1.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_A/k_2.tex <==
2

==> Experiments/Parameter_Choice/SplineOrder_A/k_3.tex <==
3

==> Experiments/Parameter_Choice/SplineOrder_B/alpha_1.tex <==
5000

==> Experiments/Parameter_Choice/SplineOrder_B/alpha_2.tex <==
5000

==> Experiments/Parameter_Choice/SplineOrder_B/alpha_3.tex <==
5000

==> Experiments/Parameter_Choice/SplineOrder_B/gamma_1.tex <==
0.1

==> Experiments/Parameter_Choice/SplineOrder_B/gamma_2.tex <==
0.1

==> Experiments/Parameter_Choice/SplineOrder_B/gamma_3.tex <==
0.1

==> Experiments/Parameter_Choice/SplineOrder_B/k_1.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_B/k_2.tex <==
2

==> Experiments/Parameter_Choice/SplineOrder_B/k_3.tex <==
3

==> Experiments/Parameter_Choice/SplineOrder_C/alpha_1.tex <==
100

==> Experiments/Parameter_Choice/SplineOrder_C/alpha_2.tex <==
100

==> Experiments/Parameter_Choice/SplineOrder_C/alpha_3.tex <==
100

==> Experiments/Parameter_Choice/SplineOrder_C/gamma_1.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_C/gamma_2.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_C/gamma_3.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_C/k_1.tex <==
1

==> Experiments/Parameter_Choice/SplineOrder_C/k_2.tex <==
2

==> Experiments/Parameter_Choice/SplineOrder_C/k_3.tex <==
3

==> Experiments/Run_Time/Run_Time_B/K_BZ.tex <==
1, 2, 3, 4

==> Experiments/Run_Time/Run_Time_B/K_Potts.tex <==
1, 2, 3, 4

==> Experiments/Run_Time/Run_Time_B/Random_Signal_Example.tex <==
\begin{figure}[t]
	\centering
\begin{subfigure}{0.24\textwidth}
	\includegraphics[width=\textwidth]{Experiments/Run_Time/Run_Time_B/Random_Signal_Example_k1.pdf}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
	\includegraphics[width=\textwidth]{Experiments/Run_Time/Run_Time_B/Random_Signal_Example_k2.pdf}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
	\includegraphics[width=\textwidth]{Experiments/Run_Time/Run_Time_B/Random_Signal_Example_k3.pdf}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
	\includegraphics[width=\textwidth]{Experiments/Run_Time/Run_Time_B/Random_Signal_Example_k4.pdf}
\end{subfigure}
		\caption{
		\label{Fig Example Random_Signal}
		Noiseless examples of the randomly generated signals used for the experiments in \cref{Figure_Experiments_RunTime_PwPoly}.
		\mar{weg damit?}{}
		%$k=1,2,3,4$ that were generated as described in \cref{Section Computing Time}. 
	}
\end{figure}

==> Experiments/Run_Time/Run_Time_B/Run_Time_B_Potts.tex <==
\begin{figure}[H]
\begin{subfigure}{0.4\textwidth}
\includegraphics[width=\textwidth]{Experiments/Run_Time/Run_Time_B/Run_Time_Potts_B.pdf}
\end{subfigure}
\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=\textwidth]{Experiments/Run_Time/Run_Time_B/Run_Time_BZ_B.pdf}
\end{subfigure}
\end{figure}

==> Experiments/Run_Time/Run_Time_B/jumpsInterval_BZ.tex <==
1

==> Experiments/Run_Time/Run_Time_B/jumpsInterval_Potts.tex <==
1

==> Experiments/Run_Time/Run_Time_B/jumps_per_segment_BZ.tex <==
1

==> Experiments/Run_Time/Run_Time_B/jumps_per_segment_Potts.tex <==
1

==> Experiments/Run_Time/Run_Time_B/maxN_BZ.tex <==
10000

==> Experiments/Run_Time/Run_Time_B/maxN_Potts.tex <==
10000

==> Experiments/Run_Time/Run_Time_B/noise_lvl_BZ.tex <==
0.1

==> Experiments/Run_Time/Run_Time_B/prob_of_jump_BZ.tex <==
0.01

==> Experiments/Run_Time/Run_Time_B/repeats_BZ.tex <==
1000

==> Experiments/Run_Time/Run_Time_B/stepSize_BZ.tex <==
100

==> Experiments/Run_Time/Run_Time_B/stepSize_Potts.tex <==
100

==> Experiments/Run_Time/Run_Time_D/nr_repeats.tex <==
10

==> Experiments/Run_Time/Run_Time_D/q_max.tex <==
17

==> Experiments/Run_Time/Run_Time_D/q_min.tex <==
9

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_A/Run_Time_Vs_Pottslab_A.tex <==
\begin{figure}[]
	\centering
\includegraphics[width=0.6\textwidth]{Experiments/Run_Time/Run_Time_Vs_Pottslab_A/Run_Time_Vs_Pottslab_A.pdf}
\caption{
	\label{Figure_Experiments_RunTime_VsPottslab_A}
	Piece length 
	$m=
	\protect\input{Experiments/Run_Time/Run_Time_Vs_Pottslab_A/stepSize.tex}
	$,
	10\% noise level. 
	For every considered $n$, we computed $
	\protect\input{Experiments/Run_Time/Run_Time_Vs_Pottslab_A/repeats.tex}
	$ instances and plotted the mean computation time.
	}
\end{figure}



==> Experiments/Run_Time/Run_Time_Vs_Pottslab_A/jumpsInterval.tex <==
2

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_A/k.tex <==
1

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_A/maxN.tex <==
10000

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_A/repeats.tex <==
2

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_A/stepSize.tex <==
100

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/RunTime_Vs_Pottslab_Table.tex <==
Comp. Time [s] & Blocks & Bumps & Heavy Sine & Doppler \\ 
\hline 
Pottslab & 0.410 & 0.315 & 0.433  & 0.338 \\ 
Toolbox & 0.041 & 0.031 & 0.020  & 0.015 \\ 
\hline 


==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/Run_Time_Vs_Pottslab_B.tex <==
\begin{table}[h]	
	\centering
\begin{tabular}{ | l | c  c  c  c |}
	\hline
\input{Experiments/Run_Time/Run_Time_Vs_Pottslab_B/RunTime_Vs_Pottslab_Table.tex}
 \end{tabular}
\caption{
	Computation times needed by Pottslab and our implementation for the classical piecewise constant Potts problem corresponding to $k=1$.
	Data are Donoho--Johnstone	 test signals of length
	$n=\protect\input{Experiments/Run_Time/Run_Time_Vs_Pottslab_B/n.tex}$
	 corrupted by Gaussian noise with noise level
$\protect\input{Experiments/Run_Time/Run_Time_Vs_Pottslab_B/noise_lvl.tex}$. 
Jump penalties were chosen according to BIC.
We repeated the reconstructions 
$\protect\input{Experiments/Run_Time/Run_Time_Vs_Pottslab_B/nr_repeats.tex}$
times and took the mean. Our implementation is at least 10 times faster facing the Donoho--Johnstone signals.
	}
\end{table}


==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/gamma_blocks.tex <==
0.53068

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/gamma_bumps.tex <==
0.078528

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/gamma_doppler.tex <==
0.0058217

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/gamma_heavysine.tex <==
0.60613

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/n.tex <==
8192

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/noise_lvl.tex <==
0.1

==> Experiments/Run_Time/Run_Time_Vs_Pottslab_B/nr_repeats.tex <==
20

==> Experiments/Synthetic_Data/Donoho_Blocks_A/MSE_BZ_1.tex <==
5.4142e-05

==> Experiments/Synthetic_Data/Donoho_Blocks_A/MSE_BZ_2.tex <==
2.1515e-05

==> Experiments/Synthetic_Data/Donoho_Blocks_A/MSE_BZ_3.tex <==
1.3205e-05

==> Experiments/Synthetic_Data/Donoho_Blocks_A/MSE_Potts_1.tex <==
1.3386e-06

==> Experiments/Synthetic_Data/Donoho_Blocks_A/MSE_Potts_2.tex <==
1.368e-06

==> Experiments/Synthetic_Data/Donoho_Blocks_A/MSE_Potts_3.tex <==
9.9121e-07

==> Experiments/Synthetic_Data/Donoho_Blocks_A/Rand_BZ_1.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Blocks_A/Rand_BZ_2.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Blocks_A/Rand_BZ_3.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Blocks_A/Rand_Potts_1.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Blocks_A/Rand_Potts_2.tex <==
0.98

==> Experiments/Synthetic_Data/Donoho_Blocks_A/Rand_Potts_3.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Blocks_A/alpha_1.tex <==
1.44

==> Experiments/Synthetic_Data/Donoho_Blocks_A/alpha_2.tex <==
3.84

==> Experiments/Synthetic_Data/Donoho_Blocks_A/alpha_3.tex <==
6.9

==> Experiments/Synthetic_Data/Donoho_Blocks_A/beta_6.tex <==
23.800

==> Experiments/Synthetic_Data/Donoho_Blocks_A/beta_max.tex <==
25

==> Experiments/Synthetic_Data/Donoho_Blocks_A/beta_min.tex <==
0.025

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_6.tex <==
0.047

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_BZ_1.tex <==
0.0025592

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_BZ_2.tex <==
0.0051185

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_BZ_3.tex <==
0.0076777

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_Potts_1.tex <==
0.0025592

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_Potts_2.tex <==
0.0051185

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_Potts_3.tex <==
0.0076777

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_max.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Blocks_A/gamma_min.tex <==
0.001

==> Experiments/Synthetic_Data/Donoho_Blocks_A/k_BZ_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Blocks_A/k_BZ_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Blocks_A/k_BZ_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Blocks_A/k_Potts_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Blocks_A/k_Potts_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Blocks_A/k_Potts_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Blocks_A/nr_steps.tex <==
1000

==> Experiments/Synthetic_Data/Donoho_Blocks_A/randi_6.tex <==
0.99

==> Experiments/Synthetic_Data/Donoho_Blocks_A/rerr_6.tex <==
0.065

==> Experiments/Synthetic_Data/Donoho_Blocks_A/rerr_BZ_1.tex <==
0.036

==> Experiments/Synthetic_Data/Donoho_Blocks_A/rerr_BZ_2.tex <==
0.023

==> Experiments/Synthetic_Data/Donoho_Blocks_A/rerr_BZ_3.tex <==
0.018

==> Experiments/Synthetic_Data/Donoho_Blocks_A/rerr_Potts_1.tex <==
0.006

==> Experiments/Synthetic_Data/Donoho_Blocks_A/rerr_Potts_2.tex <==
0.006

==> Experiments/Synthetic_Data/Donoho_Blocks_A/rerr_Potts_3.tex <==
0.005

==> Experiments/Synthetic_Data/Donoho_Bumps_A/Donoho_Bumps_A.tex <==
\begin{figure}[]
	\captionsetup[subfigure]{justification=centering}
	\centering
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Bumps_A/Bumps_Data.pdf}
		\subcaption{Noisy data}
	\end{subfigure}
	\begin{subfigure}{\figwidth}~
	\end{subfigure}
	\begin{subfigure}{\figwidth}~
	\end{subfigure}
	\\[1em]
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Bumps_A/Bumps_Potts_1.pdf}
	\subcaption{
		$(\Pc_{1,\infty,\gamma})$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_Potts_1.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_Potts_1.tex}$
	}						
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Bumps_A/Bumps_Potts_2.pdf}
	\subcaption{
		$(\Pc_{2,\infty,\gamma})$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_Potts_2.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_Potts_2.tex}$
	}								
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Bumps_A/Bumps_Potts_3.pdf}
	\subcaption{
		$(\Pc_{3,\infty,\gamma})$\\
		$\varepsilon_{\text{rel}} = 	\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_Potts_3.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_Potts_3.tex}$
	}										
	\end{subfigure}\\[1em]
	\begin{subfigure}{\figwidth}
	\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Bumps_A/Bumps_BZ_1.pdf}
	\subcaption{
		$(\Pc_{1,\beta,\gamma})$,~ $\beta=\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/alpha_1.tex}$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_BZ_1.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_BZ_1.tex}$
	}									
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Bumps_A/Bumps_BZ_2.pdf}
	\subcaption{
		$(\Pc_{2,\beta,\gamma})$,~ $\beta=\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/alpha_2.tex}$\\		
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_BZ_2.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_BZ_2.tex}$
	}											
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Bumps_A/Bumps_BZ_3.pdf}
	\subcaption{
		$(\Pc_{3,\beta,\gamma})$,~  $\beta=\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/alpha_3.tex}$\\		
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_BZ_3.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_BZ_3.tex}$
	}											
	\end{subfigure}
	\caption{
		\label{Fig Bumps}
		Reconstructions of ``Bumps''-signal from noisy data. The relative reconstruction error is denoted by $\varepsilon_{rel}$ and the Rand index concerning the quality of the segmentation is denoted by $R_\text{ind}$.
		(a) The data corrupted by Gaussian noise of level
		$\protect\input{Experiments/Synthetic_Data/Donoho_Bumps_A/noise_lvl.tex}$. (b)-(d) Higher order Potts model. (e)-(g) Higher order Mumford-Shah model.
	}
\end{figure}

==> Experiments/Synthetic_Data/Donoho_Bumps_A/MSE_BZ_1.tex <==
0.00017426

==> Experiments/Synthetic_Data/Donoho_Bumps_A/MSE_BZ_2.tex <==
7.3067e-05

==> Experiments/Synthetic_Data/Donoho_Bumps_A/MSE_BZ_3.tex <==
5.5464e-05

==> Experiments/Synthetic_Data/Donoho_Bumps_A/MSE_BZ_4.tex <==
5.9599e-05

==> Experiments/Synthetic_Data/Donoho_Bumps_A/MSE_Potts_1.tex <==
0.00019441

==> Experiments/Synthetic_Data/Donoho_Bumps_A/MSE_Potts_2.tex <==
9.5093e-05

==> Experiments/Synthetic_Data/Donoho_Bumps_A/MSE_Potts_3.tex <==
7.2179e-05

==> Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_BZ_1.tex <==
0.41

==> Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_BZ_2.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_BZ_3.tex <==
0.40

==> Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_Potts_1.tex <==
0.06

==> Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_Potts_2.tex <==
0.06

==> Experiments/Synthetic_Data/Donoho_Bumps_A/Rand_Potts_3.tex <==
0.08

==> Experiments/Synthetic_Data/Donoho_Bumps_A/alpha_1.tex <==
2.08

==> Experiments/Synthetic_Data/Donoho_Bumps_A/alpha_2.tex <==
4.8

==> Experiments/Synthetic_Data/Donoho_Bumps_A/alpha_3.tex <==
11.58

==> Experiments/Synthetic_Data/Donoho_Bumps_A/alpha_4.tex <==
15937.5

==> Experiments/Synthetic_Data/Donoho_Bumps_A/gamma_BZ_1.tex <==
0.010727

==> Experiments/Synthetic_Data/Donoho_Bumps_A/gamma_BZ_2.tex <==
0.021454

==> Experiments/Synthetic_Data/Donoho_Bumps_A/gamma_BZ_3.tex <==
0.032181

==> Experiments/Synthetic_Data/Donoho_Bumps_A/gamma_BZ_4.tex <==
0.0090708

==> Experiments/Synthetic_Data/Donoho_Bumps_A/gamma_Potts_1.tex <==
0.010727

==> Experiments/Synthetic_Data/Donoho_Bumps_A/gamma_Potts_2.tex <==
0.021454

==> Experiments/Synthetic_Data/Donoho_Bumps_A/gamma_Potts_3.tex <==
0.032181

==> Experiments/Synthetic_Data/Donoho_Bumps_A/k_BZ_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Bumps_A/k_BZ_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Bumps_A/k_BZ_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Bumps_A/k_BZ_4.tex <==
4

==> Experiments/Synthetic_Data/Donoho_Bumps_A/k_Potts_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Bumps_A/k_Potts_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Bumps_A/k_Potts_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Bumps_A/noise_lvl.tex <==
0.2

==> Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_BZ_1.tex <==
0.040

==> Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_BZ_2.tex <==
0.026

==> Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_BZ_3.tex <==
0.022

==> Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_Potts_1.tex <==
0.042

==> Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_Potts_2.tex <==
0.029

==> Experiments/Synthetic_Data/Donoho_Bumps_A/rerr_Potts_3.tex <==
0.026

==> Experiments/Synthetic_Data/Donoho_Doppler_A/Donoho_Doppler_A.tex <==
\begin{figure}[]
	\captionsetup[subfigure]{justification=centering}
	\centering
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Doppler_A/Doppler_Data.pdf}
		\subcaption{Noisy data}
	\end{subfigure}
	\begin{subfigure}{\figwidth}~
	\end{subfigure}
	\begin{subfigure}{\figwidth}~
	\end{subfigure}
	\\[1em]
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Doppler_A/Doppler_Potts_1.pdf}
	\subcaption{
		$(\Pc_{1,\infty,\gamma})$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_Potts_1.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_Potts_1.tex}$
	}			
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Doppler_A/Doppler_Potts_2.pdf}
	\subcaption{
		$(\Pc_{2,\infty,\gamma})$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_Potts_2.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_Potts_2.tex}$
	}					
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Doppler_A/Doppler_Potts_3.pdf}
	\subcaption{
		$(\Pc_{3,\infty,\gamma})$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_Potts_3.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_Potts_3.tex}$
	}					
	\end{subfigure}\\[1em]
	\begin{subfigure}{\figwidth}
	\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Doppler_A/Doppler_BZ_1.pdf}
	\subcaption{
		$(\Pc_{1,\beta,\gamma})$,~$\beta=\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/alpha_1.tex}$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_BZ_1.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_BZ_1.tex}$
	}				
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Doppler_A/Doppler_BZ_2.pdf}
	\subcaption{
		$(\Pc_{2,\beta,\gamma})$,~$\beta=\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/alpha_2.tex}$\\		
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_BZ_2.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_BZ_2.tex}$
	}						
	\end{subfigure}
	\begin{subfigure}{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Donoho_Doppler_A/Doppler_BZ_3.pdf}
	\subcaption{
		$(\Pc_{3,\beta,\gamma})$,~$\beta=\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/alpha_3.tex}$\\
		$\varepsilon_{\text{rel}} = 
		\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_BZ_3.tex}$, 
		$R_{\text{ind}} = \protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_BZ_3.tex}$
	}						
	\end{subfigure}
	\caption{
		\label{Fig Doppler}
		Reconstructions of ``Doppler''-signal from noisy data. The relative reconstruction error is denoted by $\varepsilon_{rel}$ and the Rand index concerning the quality of the segmentation is denoted by $R_\text{ind}$.
		(a) The data corrupted by Gaussian noise of level
		$\protect\input{Experiments/Synthetic_Data/Donoho_Doppler_A/noise_lvl.tex}$. (b)-(d) Higher order Potts model. (e)-(g) Higher order Mumford-Shah model.
	}
\end{figure}

==> Experiments/Synthetic_Data/Donoho_Doppler_A/MSE_BZ_1.tex <==
0.0003457

==> Experiments/Synthetic_Data/Donoho_Doppler_A/MSE_BZ_2.tex <==
0.00018662

==> Experiments/Synthetic_Data/Donoho_Doppler_A/MSE_BZ_3.tex <==
0.00012343

==> Experiments/Synthetic_Data/Donoho_Doppler_A/MSE_Potts_1.tex <==
0.00048399

==> Experiments/Synthetic_Data/Donoho_Doppler_A/MSE_Potts_2.tex <==
0.00019183

==> Experiments/Synthetic_Data/Donoho_Doppler_A/MSE_Potts_3.tex <==
0.00012693

==> Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_BZ_1.tex <==
0.50

==> Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_BZ_2.tex <==
0.94

==> Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_BZ_3.tex <==
0.85

==> Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_Potts_1.tex <==
0.01

==> Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_Potts_2.tex <==
0.05

==> Experiments/Synthetic_Data/Donoho_Doppler_A/Rand_Potts_3.tex <==
0.10

==> Experiments/Synthetic_Data/Donoho_Doppler_A/alpha_1.tex <==
2.08

==> Experiments/Synthetic_Data/Donoho_Doppler_A/alpha_2.tex <==
4.8

==> Experiments/Synthetic_Data/Donoho_Doppler_A/alpha_3.tex <==
11.58

==> Experiments/Synthetic_Data/Donoho_Doppler_A/gamma_BZ_1.tex <==
0.023519

==> Experiments/Synthetic_Data/Donoho_Doppler_A/gamma_BZ_2.tex <==
0.047038

==> Experiments/Synthetic_Data/Donoho_Doppler_A/gamma_BZ_3.tex <==
0.070558

==> Experiments/Synthetic_Data/Donoho_Doppler_A/gamma_Potts_1.tex <==
0.023519

==> Experiments/Synthetic_Data/Donoho_Doppler_A/gamma_Potts_2.tex <==
0.047038

==> Experiments/Synthetic_Data/Donoho_Doppler_A/gamma_Potts_3.tex <==
0.070558

==> Experiments/Synthetic_Data/Donoho_Doppler_A/k_BZ_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Doppler_A/k_BZ_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Doppler_A/k_BZ_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Doppler_A/k_Potts_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Doppler_A/k_Potts_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Doppler_A/k_Potts_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Doppler_A/noise_lvl.tex <==
0.2

==> Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_BZ_1.tex <==
0.063

==> Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_BZ_2.tex <==
0.046

==> Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_BZ_3.tex <==
0.038

==> Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_Potts_1.tex <==
0.075

==> Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_Potts_2.tex <==
0.047

==> Experiments/Synthetic_Data/Donoho_Doppler_A/rerr_Potts_3.tex <==
0.038

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/MSE_BZ_1.tex <==
0.00025176

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/MSE_BZ_2.tex <==
0.00011518

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/MSE_BZ_3.tex <==
5.0076e-05

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/MSE_Potts_1.tex <==
0.00014346

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/MSE_Potts_2.tex <==
3.8513e-05

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/MSE_Potts_3.tex <==
2.3023e-05

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/Rand_BZ_1.tex <==
0.84

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/Rand_BZ_2.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/Rand_BZ_3.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/Rand_Potts_1.tex <==
0.67

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/Rand_Potts_2.tex <==
0.73

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/Rand_Potts_3.tex <==
0.82

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/alpha_1.tex <==
2.08

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/alpha_2.tex <==
4.8

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/alpha_3.tex <==
11.58

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/beta_6.tex <==
23.725

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/beta_min.tex <==
0.025

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_6.tex <==
0.141

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_BZ_1.tex <==
0.016837

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_BZ_2.tex <==
0.033674

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_BZ_3.tex <==
0.050511

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_Potts_1.tex <==
0.016837

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_Potts_2.tex <==
0.033674

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_Potts_3.tex <==
0.050511

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_max.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/gamma_min.tex <==
0.001

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/k_BZ_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/k_BZ_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/k_BZ_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/k_Potts_1.tex <==
1

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/k_Potts_2.tex <==
2

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/k_Potts_3.tex <==
3

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/nr_steps.tex <==
1000

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/randi_6.tex <==
1.00

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/rerr_6.tex <==
0.030

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/rerr_BZ_1.tex <==
0.062

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/rerr_BZ_2.tex <==
0.042

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/rerr_BZ_3.tex <==
0.028

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/rerr_Potts_1.tex <==
0.047

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/rerr_Potts_2.tex <==
0.024

==> Experiments/Synthetic_Data/Donoho_Heavisine_A/rerr_Potts_3.tex <==
0.019

==> Experiments/Synthetic_Data/Gradient_Limit/Gradient_Limit.tex <==
% !TEX root = ../../../higherOrderBZ.tex
\begin{figure}[t]
	\captionsetup[subfigure]{justification=centering}	
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/Data.pdf}
	\caption*{Noisy data of piecewise smooth signal}
	\end{subfigure}\\[0.7em]
	\begin{subfigure}{0.32\textwidth}
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=1$}}}}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_1_1.pdf}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_1_2.pdf}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_1_3.pdf}
	\end{subfigure}	
	\\[0.7em]
	\begin{subfigure}{0.32\textwidth}
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=2$}}}}	
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_2_1.pdf}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_2_2.pdf}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_2_3.pdf}
	\end{subfigure}	
	\\[0.7em]
	\begin{subfigure}{0.32\textwidth}
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=3$}}}}	
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_3_1.pdf}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_3_2.pdf}
	\end{subfigure}
	\hspace{0.1cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_3_3.pdf}
	\end{subfigure}	
	\caption{``Gradient limit effect'' of classical Mumford-Shah ($k=1$): 
	}
	\label{fig:GradientLimit_big}
\end{figure}

==> Experiments/Synthetic_Data/Gradient_Limit/Gradient_Limit_small.tex <==
% !TEX root = ../../../higherOrderBZ.tex
\begin{figure}[t]
	\captionsetup[subfigure]{justification=centering}	
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/Data.pdf}
	\caption*{Noisy data of piecewise smooth signal}
	\end{subfigure}\\[0.7em]
	\begin{subfigure}{0.32\textwidth}
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=1$}}}}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_1_1.pdf}
		\caption{small $\beta$/ low smoothing level}
	\end{subfigure}
	\hspace{0.8cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_1_2.pdf}
		\caption{large $\beta$/ high smoothing level}
	\end{subfigure}
	\\[0.7em]
	\begin{subfigure}{0.32\textwidth}
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=2$}}}}	
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_2_1.pdf}
		\caption{small $\beta$/ low smoothing level}
	\end{subfigure}
	\hspace{0.8cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/MS_2_2.pdf}
		\caption{large $\beta$/ high smoothing level}
	\end{subfigure}	
	\caption{
		\emph{(a)} Applying the first order Mumford-Shah model for a small choice of $\beta$  is prone to noise.
		\emph{(b)} Calling for a higher (an acceptable/reasonable?) smoothing level (increasing $\beta$) leads to a spurious segment in the middle interval (``Gradient limit effect''), while the last discontinuity of the clean signal is smoothed out:	the denoising potential of the first order model for signals with steep slopes is limited.
		(\textbf{Noch dazu?}: Increasing/decreasing of jump penalty is no way out)
		\emph{(c,d)} Higher orders do not suffer from the gradient limit effect: they find the correct partition for both low and high smoothing levels. 
	}
	\label{fig:GradientLimit_small}
\end{figure}

==> Experiments/Synthetic_Data/Gradient_Limit/mixed_effects/Gradient_Limit_mixed.tex <==
% !TEX root = ../../../../higherOrderBZ.tex
\begin{figure}[t]
	\captionsetup[subfigure]{justification=centering}	
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/mixed_effects/MS_1_1.pdf}
	\caption{Result of $(\Pc_{1,\beta,\gamma})$ with optimal 
	$\beta,\gamma$}
	\end{subfigure}\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/mixed_effects/MS_1_3.pdf}
		\caption{Smaller complexity penalty $\gamma$}
	\end{subfigure}\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/mixed_effects/MS_1_2.pdf}
		\caption{Larger elasticity parameter $\beta$}
	\end{subfigure}\hfill
	\caption{
		Limitations of the classical Mumford-Shah model $(\Pc_{1,\beta,\gamma}).$
		\emph{(a)}~The reconstruction from \cref{fig:splineVsMS}c with the optimized parameters
		$\gamma = 0.04$, $\beta = 1.3625$
		 is displayed. It provides unsatisfactory smoothing and  detection of discontinuities.
 \emph{(b)}~Decreasing the complexity penalty (here $\gamma= 0.02$) leads to more but dislocated discontinuities.
		\emph{(c)}~Increasing the elasticity parameter (here $\beta = 3$) leads to stronger smoothing, but to spurious segments as well.
		In either case, the first order model shows the tendency to create spurious discontinuities 
		at steep slopes which is known as the gradient limit effect.
	}
	\label{fig:GradientLimit_mixedEffects}
\end{figure}

==> Experiments/Synthetic_Data/Gradient_Limit/pure_effect/Gradient_Limit_pure.tex <==
% !TEX root = ../../../higherOrderBZ.tex
\begin{figure}[t]
	\captionsetup[subfigure]{justification=centering}	
	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/pure_effect/Data.pdf}
	\caption*{Noisy data of piecewise smooth signal}
	\end{subfigure}\\[0.7em]
	\begin{subfigure}{0.32\textwidth}
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=1$}}}}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/pure_effect/MS_1_1.pdf}
		\caption{small $\beta$/ low smoothing level}
	\end{subfigure}
	\hspace{0.8cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/pure_effect/MS_1_2.pdf}
		\caption{large $\beta$/ high smoothing level}
	\end{subfigure}
	\\[0.7em]
	\begin{subfigure}{0.32\textwidth}
		\makebox[0pt][r]{\makebox[3em]{\raisebox{40pt}{\rotatebox[origin=c]{90}{$k=2$}}}}	
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/pure_effect/MS_2_1.pdf}
		\caption{small $\beta$/ low smoothing level}
	\end{subfigure}
	\hspace{0.8cm}
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Gradient_Limit/pure_effect/MS_2_2.pdf}
		\caption{large $\beta$/ high smoothing level}
	\end{subfigure}	
	\caption{
		\emph{pure effect}
	}
	\label{fig:GradientLimit_pureEffect}
\end{figure}

==> Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_1.tex <==
3.489

==> Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_2.tex <==
3.399

==> Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_3.tex <==
3.338

==> Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_4.tex <==
3.353

==> Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_5.tex <==
3.398

==> Experiments/Synthetic_Data/Polynomial_A/Polynomial_BZ_1.tex <==
\begin{figure}[H]
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_BZ_Data.pdf}
	\end{subfigure}\\[0.4em]
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_BZ_1.pdf}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_BZ_2.pdf}
	\end{subfigure}\\[1em]
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_BZ_3.pdf}
	\end{subfigure}
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_BZ_4.pdf}
	\end{subfigure}
	\caption{
		Reconstructions for different spline orders $k$. 
		Noise is Gaussian with $\sigma = 
		\protect\input{Experiments/Synthetic_Data/Polynomial_A/sigma_BZ.tex}
		$.
		Top: Uncorrupted piecewise polynomial signal.
		Mid row left:
		$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_BZ_1.tex}$,
		$\gamma=\protect\input{Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_1.tex}$,
		$\alpha=\protect\input{Experiments/Synthetic_Data/Polynomial_A/alpha_1.tex}$.
		Mid row right: 
		$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_BZ_2.tex}$,
		$\gamma=\protect\input{Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_2.tex}$,
		$\alpha=\protect\input{Experiments/Synthetic_Data/Polynomial_A/alpha_2.tex}$.
		Bottom left: 
		$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_BZ_3.tex}$,
		$\gamma=\protect\input{Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_3.tex}$,
		$\alpha=\protect\input{Experiments/Synthetic_Data/Polynomial_A/alpha_3.tex}$.
		Bottom right:
		$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_BZ_4.tex}$,
		$\gamma=\protect\input{Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_4.tex}$,
		$\alpha=\protect\input{Experiments/Synthetic_Data/Polynomial_A/alpha_4.tex}$.
	}
\end{figure}

==> Experiments/Synthetic_Data/Polynomial_A/Polynomial_Potts_1.tex <==
% !TEX root = ../../../higherOrderBZ.tex
\begin{figure}[]
	\centering
	\def\figwidth{0.32\textwidth}
	\begin{subfigure}[t]{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_Potts_Data.pdf}
		\caption{Noisy data}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_Potts_1.pdf}
		\caption{ $(\Pc_{1,\infty, \gamma}),$ BIC--score: \protect\input{Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_1.tex}
		}
	\end{subfigure}
		\hfill
	\begin{subfigure}[t]{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_Potts_2.pdf}
		\caption{
			$(\Pc_{2,\infty, \gamma}),$ BIC--score: 			
			\protect\input{Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_2.tex}
		}
	\end{subfigure}\\[1em]
	%%%%%%phantom for figure placement
		\begin{subfigure}[t]{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_Potts_3.pdf}
		\caption{$(\Pc_{3,\infty, \gamma}),$
			BIC--score: 			
			\protect\input{Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_3.tex}
		}
	\end{subfigure}
		\hfill
	\begin{subfigure}[t]{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_Potts_4.pdf}
		\caption{$(\Pc_{4,\infty, \gamma}),$
			BIC--score: 			
			\protect\input{Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_4.tex}
		}
	\end{subfigure}
		\hfill
		\begin{subfigure}[t]{\figwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Polynomial_A/Polynomial_Potts_5.pdf}
		\caption{$(\Pc_{5,\infty, \gamma}),$
			BIC--score: 			
			\protect\input{Experiments/Synthetic_Data/Polynomial_A/BIC_score_Potts_5.tex}
		}		
		\end{subfigure}
	\caption{
		\label{Fig Piecewise Polynomial}
		Reconstructions of a piecewise polynomial signal from noisy data for different orders $k$. 
		Noise is Gaussian with $\sigma = 
		\protect\input{Experiments/Synthetic_Data/Polynomial_A/sigma_Potts.tex}
		$	and the $\gamma$-parameter is chosen according to BIC. The uncorrupted true signal corresponds to the red dashed line. 
		True and computed partition are indicated at the bottom of the graphs.
		%Mid row left:
		%$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_Potts_1.tex}$. 
		The classical Potts model approximates well the signal while failing in the other parts.
		%Mid row right: 
		%$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_Potts_2.tex}$. 
		The higher order Potts models of order $k=2, 3, 4$ lead to 
		better approximations of the locally linear, quadratic, and cubic trends, respectively.
		The approximation quality saturates at around $k= 4.$ 
		The best BIC score is attained for $k=3.$
		%correctly captures the constant and linear part, but makes systematic errors in the quadratic and cubic part respectively.
		%Bottom left: 
		%$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_Potts_3.tex}$.
%		Systematic error in the last interval.
		%Bottom right: 
%		Only is able to capture the signal's structure in every interval. Additionally, all segments are correctly identified.
		%$k=\protect\input{Experiments/Synthetic_Data/Polynomial_A/k_Potts_4.tex}$
	}
\end{figure}

==> Experiments/Synthetic_Data/Polynomial_A/Rand_Potts_1.tex <==
0.83

==> Experiments/Synthetic_Data/Polynomial_A/Rand_Potts_2.tex <==
0.90

==> Experiments/Synthetic_Data/Polynomial_A/Rand_Potts_3.tex <==
0.97

==> Experiments/Synthetic_Data/Polynomial_A/Rand_Potts_4.tex <==
1.00

==> Experiments/Synthetic_Data/Polynomial_A/Rand_Potts_5.tex <==
1.00

==> Experiments/Synthetic_Data/Polynomial_A/alpha_1.tex <==
200

==> Experiments/Synthetic_Data/Polynomial_A/alpha_2.tex <==
4000

==> Experiments/Synthetic_Data/Polynomial_A/alpha_3.tex <==
40000

==> Experiments/Synthetic_Data/Polynomial_A/alpha_4.tex <==
60000

==> Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_1.tex <==
0.0017102

==> Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_2.tex <==
0.0034204

==> Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_3.tex <==
0.0051306

==> Experiments/Synthetic_Data/Polynomial_A/gamma_BZ_4.tex <==
0.0068408

==> Experiments/Synthetic_Data/Polynomial_A/gamma_Potts_1.tex <==
0.012161

==> Experiments/Synthetic_Data/Polynomial_A/gamma_Potts_2.tex <==
0.024323

==> Experiments/Synthetic_Data/Polynomial_A/gamma_Potts_3.tex <==
0.036484

==> Experiments/Synthetic_Data/Polynomial_A/gamma_Potts_4.tex <==
0.048646

==> Experiments/Synthetic_Data/Polynomial_A/gamma_Potts_5.tex <==
0.060807

==> Experiments/Synthetic_Data/Polynomial_A/k_BZ_1.tex <==
1

==> Experiments/Synthetic_Data/Polynomial_A/k_BZ_2.tex <==
2

==> Experiments/Synthetic_Data/Polynomial_A/k_BZ_3.tex <==
3

==> Experiments/Synthetic_Data/Polynomial_A/k_BZ_4.tex <==
4

==> Experiments/Synthetic_Data/Polynomial_A/k_Potts_1.tex <==
1

==> Experiments/Synthetic_Data/Polynomial_A/k_Potts_2.tex <==
2

==> Experiments/Synthetic_Data/Polynomial_A/k_Potts_3.tex <==
3

==> Experiments/Synthetic_Data/Polynomial_A/k_Potts_4.tex <==
4

==> Experiments/Synthetic_Data/Polynomial_A/k_Potts_5.tex <==
5

==> Experiments/Synthetic_Data/Polynomial_A/sigma_BZ.tex <==
0.015

==> Experiments/Synthetic_Data/Polynomial_A/sigma_Potts.tex <==
0.04

==> Experiments/Synthetic_Data/Spline_Examples/Spline_Examples.tex <==
% !TEX root = ../../../higherOrderBZ.tex
\begin{figure}[t]
%	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Spline_Examples/Data.pdf}
	\caption{Noisy signal with discontinuities}
	\end{subfigure}
\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Spline_Examples/Spline2.pdf}
		\caption{Smoothing spline}
	\end{subfigure}
\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Spline_Examples/MS_1st.pdf}
		\caption{Classical Mumford-Shah $(\Pc_{1,\beta,\gamma})$}
	\end{subfigure}\\[0.7em]
%	\centering
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Spline_Examples/MS_2nd.pdf}
		\caption{Higher order Mumford-Shah $(\Pc_{2,\beta,\gamma})$}
	\end{subfigure}\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Spline_Examples/MS_3rd.pdf}
		\caption{Higher order Mumford-Shah $(\Pc_{3,\beta,\gamma})$}
	\end{subfigure}\hfill
	\begin{subfigure}{0.32\textwidth}
		\includegraphics[width=1\textwidth,trim=25 14 0 0, clip]{Experiments/Synthetic_Data/Spline_Examples/MS_4th.pdf}
		\caption{Higher order Mumford-Shah $(\Pc_{4,\beta,\gamma})$}
	\end{subfigure}	
	\caption{
		Smoothing a noisy signal with discontinuities   using various models. All model parameters are chosen with respect to optimal $\ell^2$-error.
		The red  dashed lines depict the ground truth; the streaks at the bottom indicate the  discontinuities or segments of the ground truth (top, red) and the computed segmentations (bottom, blue).
		\emph{(b)}~Classical spline approximation smoothes out the discontinuities.
		 \emph{(c)}~The classical Mumford-Shah model allows for discontinuities, but the estimate misses most of them and the result remains noisy.
		 \emph{(d--f)}~The higher order Mumford-Shah results provide improved smoothing and segmentation.
		 In particular, the third and the fourth order models get the discontinuities of the groundtruth.
	}
	\label{fig:splineVsMS}
\end{figure}

==> Experiments/Synthetic_Data/Spline_Examples/noise_lvl.tex <==
0.1

==> Experiments/Synthetic_Data/Tuned_Example/MSE.tex <==
9.9457e-06

==> Experiments/Synthetic_Data/Tuned_Example/Rand.tex <==
1.00

==> Experiments/Synthetic_Data/Tuned_Example/Tuned_Example.tex <==
\begin{figure}[]
	\centering
	\begin{subfigure}{0.49\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Tuned_Example/Tuned_Data.pdf}
	\caption{}
	\end{subfigure}
	\begin{subfigure}{0.49\textwidth}
		\includegraphics[width=1\textwidth]{Experiments/Synthetic_Data/Tuned_Example/Tuned_Example.pdf}
	\caption{}
	\end{subfigure}
	\caption{
		\label{Fig Tuned Example}
	Reconstruction of piecewise smooth signal (b) from noisy data (a). The dotted orange curve in (b) corresponds to the ground truth and the intervals beneath illustrate the true and the computed segmentation.
We used spline order 
$k=
\protect\input{Experiments/Synthetic_Data/Tuned_Example/k.tex}
$, jump penalty
$\gamma = 
\protect\input{Experiments/Synthetic_Data/Tuned_Example/gamma.tex}
$ and elasticity
$
\beta=
\protect\input{Experiments/Synthetic_Data/Tuned_Example/alpha.tex}
$. The signal length is
$N=
\protect\input{Experiments/Synthetic_Data/Tuned_Example/n.tex}
$ and the solution was computed in
$\protect\input{Experiments/Synthetic_Data/Tuned_Example/time.tex}$ seconds.
\mar{MS: ANDERES BILD! VORSCHLAG: SIGNAL MIT DISC, SECOND ORDER SPLINE, FIRST ORDER MUMFORD-SHAH, SECOND ORDER MUMFORD-SHAH}{}
	}
\end{figure}

==> Experiments/Synthetic_Data/Tuned_Example/alpha.tex <==
150

==> Experiments/Synthetic_Data/Tuned_Example/gamma.tex <==
2

==> Experiments/Synthetic_Data/Tuned_Example/k.tex <==
3

==> Experiments/Synthetic_Data/Tuned_Example/n.tex <==
8000

==> Experiments/Synthetic_Data/Tuned_Example/noise_lvl.tex <==
0.1

==> Experiments/Synthetic_Data/Tuned_Example/rerr.tex <==
0.005

==> Experiments/Synthetic_Data/Tuned_Example/time.tex <==
0.57
